Efficient and Optimal No-Regret Caching under Partial Observation

Online learning algorithms have been successfully used to design caching policies with sublinear regret in the total number of requests, with no statistical assumption about the request sequence. Most existing algorithms involve computationally expensive operations and require knowledge of all past requests. However, this may not be feasible in practical scenarios like caching at a cellular base station. Therefore, we study the caching problem in a more restrictive setting where only a fraction of past requests are observed, and we propose a randomized caching policy with sublinear regret based on the classic online learning algorithm Follow-the-Perturbed-Leader (FPL). Our caching policy is the first to attain the asymptotically optimal regret bound while ensuring asymptotically constant amortized time complexity in the partial observability setting of requests. The experimental evaluation compares the proposed solution against classic caching policies and validates the proposed approach under synthetic and real-world request traces.

==> Journal/FLL.tex <==
As described in~\cite{kalai2005efficient}, \texttt{FLL} shares a similar update rule to \texttt{FPL}, with the vectors $(\boldsymbol{\gamma}_t)_{t\in [T]}$ being identically distributed but correlated. Precisely, initially, \texttt{FLL} generates a vector $\boldsymbol{\alpha}$ with $N$ i.i.d. uniform random variables each within the range~$[0,\eta]$, with~$\eta=\sqrt{RAT/D}$. At each time step~$t$, the decision vector of \texttt{FLL} is $\argmin_{\mathbf{x}\in \mathcal{X}} \langle \mathbf{x}, \mathbf{g}_t \rangle$, where $\mathbf{g}_t$ is the unique vector in the following set:
    \begin{align}
            \left\{ \boldsymbol{\alpha} + \mathbf{z}\cdot \eta: \; \mathbf{z} \in \mathbb{Z}^{N} \right\} \bigcap \left\{ \sum_{s=1}^{t-1} \mathbf{r}_s + \boldsymbol{b}: \; \boldsymbol{b} \in [0,\eta]^{N} \right\}.  
    \end{align}
One can then show that the decision vector of \texttt{FLL} can be formally written as, 
\begin{align}
\mathbf{x}_{t+1} (\texttt{FLL}) = M(\boldsymbol{\alpha} + \eta \cdot \mathbf{z}(t)) :\;
 \mathbf{z}(t) = \ceil*{\frac{\mathbf{r}_{1:t} - \boldsymbol{\alpha}}{\eta}},
\end{align}
Observe that \texttt{FLL} with $\mathcal{X}$ in~\eqref{eq:Capped-Simplex} and~$\mathcal{B}$ in~\eqref{eq:requests_set} ($B=1$) coincides with the caching policy \texttt{NFLL} in the full observation setting. Using~\cite[Thm. 1.1 and Lem. 1.2]{kalai2005efficient}, we derive the regret bound~$2\sqrt{2CT}$ for \texttt{NFLL}. 



\paragraph{\texttt{NFLL}} Similarly, the computationally demanding operation is finding the $C$ items with the largest entries in the vector~$\mathbf{m}$. The latter has the property that at most one of its components is updated at each step, which allows to employ a heap to keep track of the top~$C$ and incurring a time complexity of~$\mathcal{O}(\ln{C})$ per insertion/deletion. At each time step~$t$, the component $f_t$ of the vector $\mathbf{m}$ is updated if and only if the quantity $\ceil*{\frac{\hat n_{f_t}(t)-\alpha_{f_t}}{\eta^{'}}}-\ceil*{\frac{\hat n_{f_t}(t-1)-\alpha_{f_t}}{\eta^{'}}}$, denoted $\Delta_t$, is larger or equal to~$1$. Consequently, the average number of insertions and deletions is proportional to $\sum_{t=1}^{T}\Proba{\Delta_t=1}$. We prove that~$\Proba{\Delta_t=1}\leq pq/\eta^{'}$, with $\eta^{'}= \sqrt{T/2C}$, to deduce that the average amortized time complexity of \texttt{NFLL} is~$\mathcal{O}(1+\ln(C)\sqrt{C}/\sqrt{T})$.   

Only the componenent correponding to the requested file at step~$t$, $f_t$, of the noise vector is updated from step $t-1$ to step $t$, i.e., 

For the lazy variant of \texttt{NFPL}, 
    \begin{align}
             \Delta_{t}(f,\texttt{L}) = \begin{cases}
                    \eta ,&\text{ if } f= f_t, \; t\%B = 0  \;  \\ 
                    0  ,&\text{ otherwise}.
                       \end{cases} 
    \end{align}





the sets of cached items at step~$t$ and~$t-1$ differ by at most one file, i.e., $|S_t\setminus S_{t-1}|\leq 1$, which enables to dynamically keep track of the top~$C$ files via a \textit{heap} data structure (ordered binary tree). The latter updates 

returns the file with lowest perturbed count in $S_{t-1}$ in $\mathcal{O}(1)$   






All variants store at each time step~$t$, the~$C$ files with the largest~$\hat{n}_{f}(t) + \gamma_{t,f}$, for $f\in \mathcal{I}$. Let $\Delta_t(f,\mathcal{A})$ be the change of this quantity from step~$t-1$ to~$t$ when using the variant $\mathcal{A}$ of \texttt{NFPL}, i.e., 
\begin{align}
        \Delta_{t}(f,\mathcal{A}) = \hat{n}_{f}(t) + \gamma_{t,f} - \hat{n}_{f}(t-1) + \gamma_{t-1,f}. 
\end{align}

==> Journal/Recovery_Files/analysis.tex <==
The proof employs similar techniques used in the original paper of FPL \cite{kalai2005efficient}. Which makes use of the virtual policy that considers costs up to time $t$ at time step $t$. 

\begin{align}
    \widehat{\text{NBPL}}(1:T) = \sum_{t=1}^{T} \hat r_t \cdot M(\hat r_{0:t}).
\end{align}
For convenience, we define $\hat{\text{NFPL}}$ as the policy that takes the same decision as NFPL but the cost is also evaluated with respect to the noisy costs $\hat r_t$. More specifically: 
    \begin{align}
        &\widehat{\text{NFPL}}(1:T) = \sum_{t=1}^{T} \hat r_t \cdot M(\hat r_{0:t-1}).
    \end{align}
\color{blue}
\begin{lemma} \label{lem:hat-NFPL-NFPL}
NFPL and $\widehat{\text{NFPL}}$ have the same expected cost. 

\begin{equation}
    \Ex{\text{NFPL}}{\{\hat r_s\}_{0}^{T}} =   \Ex{\widehat{\text{NFPL}}}{\{\hat r_s\}_{0}^{T}} .   
\end{equation}
\color{black}
\begin{proof}
The random vectors $\hat r_t$ and $M(\hat r_{0:t-1})$ are independent, by linearity of the expectation, the result follows. 
\end{proof}
\end{lemma}


\color{black}
% \begin{remark}
%     The previous lemma is not valid for NBPL because $\hat r_t$ and $M(\hat r_{0:t})$ are clearly dependent. 
% \end{remark}

% \begin{lemma}
% $\hat{\text{NBPL}}$ is not that far from the static optimum 
% \begin{align}
%     \Ex{\hat{\text{NBPL}}}{\{r_s\}_{0}^{T}} \leq \text{OPT}(1:T) + \Ex{\hat r_0 \cdot (M(\hat r_{1:T})  - M(\hat r_0))}{r_s}
% \end{align}
% \begin{proof}
% Make use of the fact that: 
%     \begin{align}
%         \sum_{t=0}^{T} y_t \cdot M(y_{0:t}) \leq y_{0:T} M(y_{0:T}) 
%     \end{align}
% for any vectors $y_t$, it is proven in \cite{kalai2005efficient}. 
% \end{proof}
% \end{lemma}



% \begin{lemma}

% \begin{align}
%     \Ex{\hat r_0 \cdot (M(\hat r_{1:T})  - M(\hat r_0))}{r_s} \leq \eta \cdot D_1 
% \end{align}
 
% \end{lemma}

\color{blue}
\begin{lemma}\label{lem:hatNBPL-OPT}
\begin{align}
    \Ex{\widehat{\text{NBPL}}}{\hat \{r_s\}_{0}^{T}} \leq \text{OPT}(1:T) + \eta \cdot D_1 .
\end{align}
\color{black}
\begin{proof}
Make use of the fact that: 
    \begin{align}
        \sum_{t=0}^{T} y_t \cdot M(y_{0:t}) \leq y_{0:T} M(y_{0:T}) 
    \end{align}
for any vectors $y_t$, it is proven in \cite{kalai2005efficient}. For $y_t= \hat r_t$ we get: 

\begin{align}
     \sum_{t=0}^{T} \hat r_t \cdot M(\hat r_{0:t})
     &\leq \hat r_{0:T} M(\hat r_{0:T}) \\
     & \leq \hat r_{0:T} M(\hat r_{1:T}) \\ 
     & = \hat M(\hat r_{1:T})( \hat  r_{1:T} + \hat r_{0}) .
\end{align}
It follows that: 
\begin{align}
 \widehat{\text{NBPL}} 
 &=    \sum_{t=1}^{T} \hat r_t \cdot M(\hat r_{0:t}) \\
&\leq \hat r_{1:T} \cdot M(\hat r_{1:T})    + \hat r_0 \left( M(\hat r_{1:T}) - M(\hat r_0)\right)  \\ 
&\leq \hat r_{1:T} \cdot M(r_{1:T})+ \hat r_0 \left( M(\hat r_{1:T}) - M(\hat r_0)\right).
\end{align}
Taking the expectation over $\{\hat r_s\}_{0}^{T}$ and using Lemma 6 in \cite{RobertNotes} we get the desired result.

\end{proof}
\end{lemma}
\color{black}
\color{blue}
\begin{lemma}\label{lem:shifted-uniform-coupling}
Let $X$ be random vector with probability distribution $p$ over $\mathds{R}^{N}$, where each component is a uniform distribution in $[a_i,b_i]$,   $a,b\in \mathds{R}^{N}\times \mathds{R}^{N}$,$b_i-a_i = 2\eta >0$,  and the realization of each component is independent from the others. Let $Y$ be random variable with the same probability distribution as $X+r$, we call it $q$, where $r\in \mathds{R}^{N}$ such that $a+r<b$. There exist a coupling between $X$ and $Y$, $Z=(X,Y)$ such that: 
\begin{equation}
    \Proba{X \neq Y} \leq \frac{\norm{r}_1}{2\eta} .
\end{equation}
\color{black}
\begin{proof}
 We consider 
 
 \begin{equation}
     Y = \begin{cases}
      X &\text{ if }   a + r \leq  X \leq b\\
      X+ b-a &\text{otherwise}.
    \end{cases}
 \end{equation}
It is easy to check that if $X$ has distribution $p$ then $Y$ with the construction above has also distribution $q$. Moreover, 

\begin{align}
    \Proba{X\neq Y} 
&= \Proba{\exists i \in [N]:\; a_i \leq X_i \leq a_i + r_i } \\
&\leq \sum_{i=1}^{N} \Proba{ a_i \leq X_i \leq a_i + r_i} \\ 
&=  \sum_{i=1}^{N} r_i \cdot \frac{1}{b_i-a_i} \\
&\leq \frac{\norm{r}_1}{2\eta}\ .
\end{align}
\end{proof}
\end{lemma}
\color{blue}

\begin{lemma}\label{lem:NFPL-NBPL}
For any realization of $\{ \hat r_s\}_{1}^{T}$
    \begin{align}
        \Ex{\widehat{\text{NFPL}}}{\{\hat r_s \}_{1}^{T}} \leq \Ex{\widehat{\text{NBPL}}}{\{\hat r_s \}_{1}^{T}} + R \cdot \frac{B}{p} \cdot \frac{T}{2 \eta} \ .
    \end{align}
\color{black}
    \begin{proof}
    Follows directly from \cite{RobertNotes} Corollary 4 and Lemma 5, by considering the costs vector to be $\{\hat r_s\}_{1}^{T}$ and noticing that $\norm{\hat r_t}_1 \leq \frac{B}{p}$. The only problem is that there is a mistake in the proof of Lemma 5. More details: 
    \begin{align}
        \Ex{\widehat{\text{NFPL}} - \widehat{\text{NBPL}}}{\hat r_0}
&= \sum_{t=1}^{T} \hat r_t \cdot \Ex{M(\hat r_{0:t-1}) -M(\hat r_{0:t}) }{\hat r_0}
    \end{align}
$\hat r_{0:t-1}$ is are  uniform distribution $\hat r_{0:t}$ has a distribution of $\hat{r_{0:t-1}} + r_t$. Using Lemma \ref{lem:shifted-uniform-coupling}, we can find two random vectors $y_1$ and $y_2$ with the same distribution as $\hat r_{0:t-1}$ and $\hat r_{0:t}$, respectively. Moreover we have:   

\begin{align}
     \Proba{y_1 \neq y_2} \leq \frac{B}{p} \cdot \frac{1}{2 \eta} ,
\end{align}

\begin{align}
    &\hat r_t\cdot \Ex{M(\hat r_{0:t-1}) -M(\hat r_{0:t}) }{\hat r_0}\nonumber\\
    &= \hat r_t\cdot \Ex{M(y_1)-M(y_2)}{(y_1,y_2)} \\\nonumber
    & =\hat r_t \cdot( \Ex{M(y_1)-M(y_2)\mid y_1 = y_2}{(y_1,y_2)} \mu (y_1=y_2) \\ 
    &\;\;\;+  \Ex{M(y_1)-M(y_2)\mid y_1 = y_2}{(y_1,y_2)} \mu (y_1\neq y_2) )\\
    & = \hat r_t \cdot \Ex{M(y_1)-M(y_2)\mid y_1 = y_2}{(y_1,y_2)} \mu (y_1\neq y_2) \\ 
    &\leq R \cdot \frac{B}{p}\cdot \frac{1}{2\eta} \ .
\end{align}
By taking the expectation over $\{\hat r_s \}_{1}^{T}$ and then summing from $t=1$ to $T$, we get the desired result.
\end{proof}
\end{lemma}


\begin{proof}[Theorem 3] 
Simply combining Lemmas \ref{lem:hat-NFPL-NFPL}, \ref{lem:hatNBPL-OPT}, \ref{lem:NFPL-NBPL}. 
\end{proof}
\color{black}

==> Journal/Recovery_Files/approach1.tex <==
\subsection{FPL with noisy costs}


\begin{algorithm}[h] 
\KwIn{Set of decisions $\mathcal{X}$; Time Horizon $T$; $R, \; A, \; D$}
\KwOut{Sequence of decisions: $\{x_t\}_{1}^{T}$}

$\eta \gets \sqrt{\frac{R\cdot A \cdot T}{D}}$ \\ 
$\hat{\textbf{costs}} \gets  0$ ,  \\ 
\For{round $t=1,2,...,T$}{
$\mathbf{x_t} \gets M(\hat{\textbf{costs}} +  \textbf{Unif}\left(\left[0, \eta\right], \mathbb{I}_{N\times N}\right))$ \\ 
Observe $\hat{\mathbf{r_t}}$ \\
$\hat{\textbf{costs}} \gets \hat{\textbf{costs}} + \hat{r_t}$
}
\label{alg:NFPL}
\caption{Noisy Follow the Perturbed Leader with Uniform Noise (NFPL)}
\end{algorithm}


Our main contribution is proposing a more general version of the FPL algorithm where we do not have necessarily access to the exact cost vector, $r_t$, but only to its estimation: $\hat r_t$. $\hat r_t$ is an unbiased estimator of $r_t$ with bounded $l_1$ norm for every realization, i.e. 

\begin{align}
   \E{\hat r_t} = r_t , \; \sup_{t\in [T],\; \omega \in \Omega} \norm{\hat r_t (\omega)}_1 \leq A  
\end{align}
and $\norm{x}_1 = \sum_{i=1}^{N} \|x_i\|$ 
Our proposed algorithm $1$, we call it Noisy Follow the Perturbed Leader (NFPL),  follows the same procedure as FPL with uniform noise but using at each time step, the estimation $\hat r_t$ instead of the real cost vector $r_t$. Algorithm $1$ is not specific to the caching problem but more general to any online learning problem. More specifically, the set of decisions $\mathcal{X}$ could be any other compact set with $l_1$ diameter $D = \sup_{x,y \in \mathcal{X}} \norm{x-y}_{1}$. The set $\bar{\mathcal{B}}$ of costs could be any other with bounded $l_1$ norm for every one of its elements, 

The operation $M(\textbf{costs})$ corresponds   

\begin{align}
    &R = \sup_{x\in \mathcal{X}, t\in [T]} \scalar{r_t}{x}\\
    &D= \sup_{x,y \in \mathcal{X}} \norm{x-y}_{1} \\ 
    &A = \sup_{r\in \bar{\mathcal{B}}} \norm{r}_{1} 
\end{align}
\begin{theorem}[Regret bounds NFPL]
For $\eta = \sqrt{\frac{R\cdot A \cdot T}{D_1}}$, the expected regret of NFPL verifies: 
        \begin{align}
                 \Ex{  \mathcal{R}_{T}(\text{NFPL}) }{\{\hat r_t\}_{0}^{T}}\leq 2 \sqrt{R\cdot A \cdot D\cdot T}
        \end{align}
    where the expectation is taken over the randomness of $\{\hat r_t\}_{0}^{T}$.
    


\end{theorem}

\begin{IEEEproof}
   The cost of NFPL is given by: 
    \begin{align}
        \text{NFPL}_{T} = \sum_{t=1}^{T} \scalar{r_t}{ M(\hat r_{0:t-1})}\ .
    \end{align}
We similarly define the policy $\hat{\text{NFPL}}$ that plays the same actions as NFPL for a given $\{\hat r_t\}_{0}^{T}$ but evaluated with respect to the noisy requests, instead of the actual requests, more specifically its cost is given by: 

\begin{align}
   \hatname{NFPL}_{T} = \sum_{t=1}^{T} \scalar{\hat r_t} {M(\hat r_{0:t-1})} , \hat{\text{OPT}}_{T} = \scalar{\hat r_{1:T}}{M(\hat r_{1:T})}  \ . 
\end{align}
the regret can be written as: 
\begin{align}
    &\E{\mathcal{R}_{T}(\text{NFPL})} \\
&= \E{\text{NFPL}_{T} - \text{OPT}_{T}} \\ 
&= \E{\text{NFPL}_{T} - \hatname{NFPL}_{T}} + \\
&\;  \E{\hatname{NFPL}_{T} - \hatname{OPT}_{T}} + \E{ \hatname{OPT}_{T} -\text{OPT}_{T}}
\end{align}
We have: 
\begin{align} \label{e:proof-NFPL1}
    &\E{\text{NFPL}_{T} - \hatname{NFPL}_{T}} =0\\ \label{e:proof-NFPL2}
    &\E{\hatname{OPT}_{T}-\text{OPT}_{T}} \leq 0 \\ \label{e:proof-NFPL3}
    &\E{\hatname{NFPL}_{T} - \hatname{OPT}_{T}} \leq 2\sqrt{R\cdot D\cdot A} \times \sqrt{T} 
\end{align}
The equality \eqref{e:proof-NFPL1} follows from the estimation of the noisy estimate at each time step being independent, then $\hat r_t$ and $\hat r_{0:t-1}$ are independent. The inequality \eqref{e:proof-NFPL2} is because $\hatname{OPT}\leq \hat r_{1:T} M(r_{1:T}) $. The inequality \eqref{e:proof-NFPL3} follows from \cite[Theorem 1.1]{kalai2005efficient}. 
\end{IEEEproof}







\subsection{FPL for caching with exact requests}
We deduce the following corollary as a particular deterministic estimator, the real cost vector $r_t$.  

\begin{corollary} [Regret bounds FPL caching] \label{th:FPL-uniform-noise}
For $~\eta= B \sqrt{\frac{T}{2C}}$, FPL with uniform noise applied to caching has the following regret bounds
\begin{align}
          \E{  \mathcal{R}_{T}(\text{FPL}) }
& \leq 2\sqrt{2}\cdot  B \cdot \sqrt{C \cdot T}\ .
\end{align}
\end{corollary}
\begin{IEEEproof}
It is easy to show that the $l_1$ diameter of $\mathcal{X}$ $D_1 = 2\cdot C$ and the $l_2$ diameter is given by $D_2 = \sqrt{2\cdot C}.$, The batch size is fixed hence $\norm{r_t}_{1}=B$ and $ \norm{r_t}_2 \leq B$.  $ R = \sup_{t,x} r_t x$ then $R\leq B$. Then by applying Theorem (X) from \cite{kalai2005efficient} we get our result. 
\end{IEEEproof}
For the problem of caching, \cite{bhattacharjee2020fundamental} proposes FPL algorithm for caching with a Gaussian Noise. They prove the following regret bound. 

\begin{theorem}\cite[Theorem 3]{bhattacharjee2020fundamental}
\label{th:FPL-gaussian-noise}
  For $\eta = \frac{1}{4\pi (\ln N)^{1/4}} \cdot \sqrt{\frac{T}{C}}$ and for $\gamma_t$ normal gaussians. $r_0 = \eta \cdot \gamma_t$. The expected regret of FPL is given by: 
  \begin{align}
      \E{  \mathcal{R}_{T}(\text{FPL}) } \leq 1.51 \cdot (\ln N)^{1/4} \cdot \sqrt{C\cdot T}\ .
  \end{align}
\end{theorem}

Our analysis has advantage over state of the art FPL algorithm for caching in two dimensions. First, our bounds are also valid when requests are batched, which is of practical interest, since updating the cache at each time step might be unfeasible due to the high request rate. Second, even for the case when the batch size $B=1$, our regret bounds are tighter for a catalogue size $N\geq 13$. Moreover, \cite{bhattacharjee2020fundamental} bounds diverge as $N$ goes to infinity in contrast with our bounds that are independent of the catalogue size.


















\subsection{FPL for caching with noisy requests estimates}
For the caching problem, it is of interest to consider only a subset of requests at each batch of size $l<B$. This is beneficial as the rate by which counters are updated is smaller and hence it can be afforded to use a slower cheaper memory for storing counts for each object. We consider then the setting where we have access a sample $l$ out of $B$ requests, chosen uniformly at random from the batch. If $s_t$ is the sequence of requests in the batch, with frequency count for each object inside the batch $r_t$, $\hat s_t$ is sub-sequence of $s_t$ with length $l<B$ and $\hat d_t$ is the frequency count for each object inside the batch $\hat s_t$ . The unbiased estimator in this case is given by:         

\begin{equation}\label{e:fixed-batch}
    \hat r_t  =   \frac{B}{l} \cdot \hat d_t: \; \E{\hat r_t} = r_t, \; \sup_{t\in [T],\; \omega \in \Omega} \norm{\hat r_t(w)}_{1} = B
\end{equation}



    

\begin{corollary}[Regret Bounds NFPL with fixed size sub-batch]\label{co:NFPL-caching-fixed-subBatch}
      For $\eta = B \cdot \sqrt{\frac{T}{2\cdot C}}$, the expected regret of NFPL verifies: 
        \begin{align}
                 \E{  \mathcal{R}_{T}(\text{NFPL}) }\leq 2\sqrt{2} \cdot B \cdot \sqrt{C\cdot T}
        \end{align}
\end{corollary}

Another model, is to consider a sub-batch that samples each request with a probability $f>0$ at each time step, in this case the size of the batch is a random variable and the unbiased estimator $\hat r_t$ is expressed in this case as: 

\begin{equation}
    \hat r_t = \frac{1}{p} \cdot \hat d_t 
\end{equation}


\begin{corollary}[Regret Bounds NFPL sampling probability $f$]
      For $\eta = B \cdot \sqrt{\frac{T}{2\cdot C}}$, the expected regret of NFPL verifies: 
        \begin{align}
                 \E{  \mathcal{R}_{T}(\text{NFPL}) }\leq 2\sqrt{2} \cdot \frac{B}{f} \cdot \sqrt{C\cdot T}
        \end{align}
        
    \begin{IEEEproof}
        The proof follows from Theorem $1$ and noticing that $\norm{\hat r_t} \leq \frac{B}{f}$  
    \end{IEEEproof}
\end{corollary}

\begin{remark}
It is possible to prove the tighter bound without dependency on $f$ but I think it will require refering to results inside the notes of Kleinberg, maybe it is not worth it ? 
\end{remark}


% \begin{remark}
%  It seems that the difference between NFPL and FPL is the constant in the regret $\frac{1}{p}$. But NFPL has more variance, since the expectation is taken now over more randomness. 
% \end{remark}



% \begin{algorithm}[h] 
% \KwIn{$R,\; T,\; B, \; D_1$}
% \KwOut{Sequence of cached items: $\{x_t\}_{1}^{T}$}

% $\eta \gets \sqrt{\frac{R\cdot B \cdot T}{D_1}}$ \\ 
% $\textbf{costs} \gets \textbf{Unif}\left(\left[0, \eta\right], \mathbb{I}_{N\times N}\right)$ ,  \\ 
% \For{round $t=1,2,...,T$}{
% $x_t \gets M(costs)$ \\ 
% Observe sample $\hat r_t \sim \frac{1}{f} \textbf{Binom}(r_t,f,\mathbb{I}_{N\times N})$ \\
% $\textbf{costs} \gets \textbf{costs} + \hat r_t$
% }
% \label{alg:NFPL}
% \caption{Follow the Perturbed Leader with Uniform Noise (NFPL) for Caching}
% \end{algorithm}
% {\noindent}Algorithm \ref{alg:NFPL} only observes a sample of requests $\hat r_t$ such that each request is seen with probability $p$. This results in noisy frequency count.

==> Journal/Recovery_Files/approach2.tex <==
%\subsection{FPL with noisy costs}
\begin{algorithm}[t]
\KwIn{Set of decisions $\mathcal{X}$; Time Horizon $T$; $R, \; A, \; D$}
\KwOut{Sequence of decisions: $\{\mathbf{x_t}\}_{1}^{T}$}

$\eta \gets \sqrt{\frac{R\cdot A \cdot T}{D}}$ \\ 
$\hat{\textbf{costs}} \gets  0$ ,  \\ 
\For{round $t=1,2,...,T$}{
$\boldsymbol{\gamma}_t \sim \textbf{Unif}\left(\left[0, \eta\right]^{N}, \mathbb{I}_{N\times N}\right)$ \\
$\mathbf{x_t} \gets M(\hat{\textbf{costs}} +  \boldsymbol{\gamma}_t)$ \\ 
Observe $\hat{\mathbf{r_t}}$ \\
$\hat{\textbf{costs}} \gets \hat{\textbf{costs}} + \mathbf{\hat{r}_{t}}$
}
\caption{Noisy Follow the Perturbed Leader with Uniform Noise (NFPL)}
\label{alg:NFPL}
\end{algorithm}

In this section we introduce an extension to the general FPL algorithm, named \textit{Noisy Follow the Perturbed Leader} (NFPL), that does not have necessarily access to the exact cost vector $\mathbf{r}_t \in \bar{\mathcal{B}}$, but only to its estimation given by a general estimator $\mathbf{\hat r}_t$. We assume that $\mathbf{\hat r}_t$ is unbiased with bounded $l_1$ norm for every realization, i.e.,
%Our main contribution is proposing a more general version of the FPL algorithm where we do not have necessarily access to the exact cost vector, $r_t$, but only to its estimation: $\hat r_t$. $\hat r_t$ is an unbiased estimator of $r_t$ with bounded $l_1$ norm for every realization, i.e. 
\begin{align}
   \E{\mathbf{\hat r}_t} = \mathbf{r}_t , \; \exists \hat A \in \mathbb{R}^+ \; \text{s.t.} \; \sup_{\mathbf{\hat r} \in \mathcal{\hat B}} \norm{\mathbf{\hat r} (\omega)}_1 \leq \hat A,
\end{align}
%G: we could try to improve the names of the constants. For me it would be natural to have R for the bound on the requests and perhaps C for the scalar product r x which corresponds to the cost.
where, $\norm{\mathbf{r}}_1 = \sum_{i=1}^{N} |r_i|$, and $\mathcal{\hat B} \subseteq \mathbb{R}^N$ is the set of all the realizations of every possible vector in the cost set $\bar{\mathcal{B}}$. %all $\mathbf{r} \in \bar{\mathcal{B}}$, where $\bar{\mathcal{B}}$ is the set of all costs. %$\mathcal{\hat B} = \{\mathbf{\hat r}_t(\omega) : \omega \in \Omega\}$ where $\Omega$ is the set of all the realizations of $\mathbf{\hat r}_t$. 
To clearly describe the algorithm we also need to introduce the definition of the upper bound of the cost, and the diameter of the decision set $\mathcal{X} \subseteq \mathbb{R}^N$ as
\begin{align}
    &\hat R = \sup_{x\in \mathcal{X}, r \in \mathcal{\bar{\hat{B}}}} \scalar{r}{x},\\
    %G: \bar{\hat{B}} is not defined, should it be \hat{B}?
    &D= \sup_{x,y \in \mathcal{X}} \norm{x-y}_{1}.
%    &A = \sup_{r\in \bar{\mathcal{B}}} \norm{r}_{1} 
\end{align}

We highlight that NFPL is not specific just to online caching, but it can deal with any general online linear learning problem. %Indeed, as described in Algorithm~\ref{alg:NFPL}, NFPL receives in input the set of decisions $\mathcal{X}$ that can be any compact subset of $\mathbb{R}^N$ with $l_1$ diameter $D$. %; iii) the upper bound $A$ on the norm of any realization of the request estimator; iv) the upper bound $R$ on the cost and v) the diameter $D$ of the decision set. 
As described in Algorithm~\ref{alg:NFPL}, NFPL follows in the footsteps of FPL with uniform noise, but considers the estimation from $\mathbf{\hat r}_t$ instead of the real cost vector $\mathbf{r}_t$. In particular, at each time-slot $t$, the algorithm generates $\boldsymbol{\gamma}_t$ from a multivariate uniform distribution in $[0, \eta]^N$, and it updates the decision vector with the minimizer of $\scalar{\mathbf{x}}{\mathbf{\hat r}_{1:t-1} +  \boldsymbol{\gamma}_t}$ over $\mathbf{x} \in \mathcal{X}$. %, where $\hat{\textbf{costs}} = \mathbf{\hat r}_{1:t-1}$.  %Once the estimation is observed, the algorithm updates the cumulative cost. %with the estimation $\mathbf{\hat r}_t$. 
%We want to highlight that NFPL is not specific to the caching problem but it can deal with any general online learning problem. More specifically, the set of the decisions $\mathcal{X}$
%Our proposed algorithm $1$, we call it Noisy Follow the Perturbed Leader (NFPL),  follows the same procedure as FPL with uniform noise but using at each time step, the estimation $\hat r_t$ instead of the real cost vector $r_t$. Algorithm $1$ is not specific to the caching problem but more general to any online learning problem. More specifically, the set of decisions $\mathcal{X}$ could be any other compact set with $l_1$ diameter $D = \sup_{x,y \in \mathcal{X}} \norm{x-y}_{1}$. The set $\bar{\mathcal{B}}$ of costs could be any other with bounded $l_1$ norm for every one of its elements, 

The performance of NFPL in terms of regret, as defined in~\eqref{eq:pseudoregret}, is expressed by the following theorem. 
\begin{theorem}[Regret bound NFPL]
For $\eta = \sqrt{\frac{R\cdot A \cdot T}{D}}$, the expected regret of NFPL verifies: 
        \begin{align}
                 \bar{\mathcal{R}}_{T}(\text{NFPL}) \leq 2 \sqrt{\hat R\cdot \hat A \cdot D\cdot T}
        \end{align}
\end{theorem}

\begin{IEEEproof}
Let $\{r_t\}_{0}^{T}$ be sequence of costs and $\{\hat{r_t}\}_{0}^{T}$ a realization from the unbiased estimator.
   The cost of NFPL given $\{r_t\}_{0}^{T}$ and $\{\hat{r_t}\}_{0}^{T}$ is expressed as: 
    \begin{align}
        \text{NFPL}_{T} = \sum_{t=1}^{T} \scalar{r_t}{ M(\hat r_{0:t-1})}\ .
    \end{align}
We similarly define the policy $\hat{\text{NFPL}}$ that plays the same actions as NFPL,  but evaluated with respect to the noisy costs, more specifically its cost is given by: 

\begin{align}
   \hatname{NFPL}_{T} = \sum_{t=1}^{T} \scalar{\hat r_t} {M(\hat r_{0:t-1})}   \ . 
\end{align}
We define also $\hat{\text{OPT}}$, the minimum cost incurred under sequence $\{\hat{r_t}\}_{0}^{T}$ given by: 
\begin{align}
    \hat{\text{OPT}}_{T} = \scalar{\hat r_{1:T}}{M(\hat r_{1:T})}
\end{align}
We compute the regret of NFPL as follows:
%G: this is wrong (I had already written it on the pages I gave to Younes), the supremum is missing. You need to say that you do the calculation for a specific sequence r_t and then take the expectation
\begin{align}
    &\bar{\mathcal{R}}_{T}(\text{NFPL}) \\
&= \E{\text{NFPL}_{T} - \text{OPT}_{T}}  \\ 
&= \E{\text{NFPL}_{T} - \hatname{NFPL}_{T}} + \\
&\;  \E{\hatname{NFPL}_{T} - \hatname{OPT}_{T}} + \E{ \hatname{OPT}_{T} -\text{OPT}_{T}}
\end{align}
We have: 
\begin{align} \label{e:proof-NFPL1}
    &\E{\text{NFPL}_{T} - \hatname{NFPL}_{T}} =0\\ \label{e:proof-NFPL2}
    &\E{\hatname{OPT}_{T}-\text{OPT}_{T}} \leq 0 \\ \label{e:proof-NFPL3}
    &\E{\hatname{NFPL}_{T} - \hatname{OPT}_{T}} \leq 2\sqrt{\hat R\cdot \hat A\cdot D} \times \sqrt{T} 
\end{align}
The equality \eqref{e:proof-NFPL1} follows from the estimations of the noisy cost at each time step being independent, then in particular $\hat r_t$ and $\hat r_{0:t-1}$ are independent and thus $\E{\scalar{\hat r_t}{M(\hat r_{0:t-1})} } = \scalar{r_t}{M(\hat r_{0:t-1})}$. The inequality \eqref{e:proof-NFPL2} is because $\hatname{OPT}\leq \hat r_{1:T} M(r_{1:T}) $. The inequality \eqref{e:proof-NFPL3} follows from \cite[Theorem 1.1]{kalai2005efficient}. 
\end{IEEEproof}

\begin{remark}
FPL algorithm for online linear learning as presented in \cite{kalai2005efficient} has a regret
%G: is this expected regret or pseudo-regret? the relation with what is discussed here it unclear. is kalai2005efficient about FPL with known costs? If so, we should not say that we do worse as our constants boil down to theirs and we recover their result.
bound of $2\cdot \sqrt{R\cdot A \cdot D\cdot T}$ where $R =\sup_{x\in \mathcal{X}, r \in \mathcal{B}} \scalar{r}{x} $ and $A = \sup_{r\in \mathcal{B}}$.
%G: the definition of A is incomplete
It is easy to check that $\hat A\geq A$ and $\hat R \geq R$. It follows that the bound for FPL would be tighter than the one we proved. The trade-off is expressed by the ratio $\sqrt{\frac{\hat R \cdot \hat A }{R \cdot A}}$. 
\end{remark}

We now study three specific cases of the unbiased estimator in the online caching setting: i) $\mathbf{\hat r}_t = \mathbf{r}_t$, i.e., the estimator is deterministic and always correct in Section~\ref{ss:FPL-caching}; 
ii) the case where a fixed number of requests is sampled within each batch and  iii) the case where each request is sampled with a given probability in Section~\ref{ss:NFPL-Caching-Fixed}. 

\subsection{FPL for caching}
\label{ss:FPL-caching}
In the online caching problem, the case where $\mathbf{\hat r}_t = \mathbf{r}_t$ translates in dealing with the exact file requests. The following result applies to the online caching problem with batched requests. 
%We consider a particular case to adapt Algorithm~\ref{alg:NFPL} for the batched caching problem. The decisions set and the costs set will be as defined in Section~\ref{sec:bacground}. Moreover, we consider the deterministic case where the estimator $\hat{\mathbf{r_{t}}}$ is always exact, i.e. $\hat{\mathbf{r_t}} = \mathbf{r_t}$. We deduce then the following result: 
\begin{corollary} [Regret bound FPL caching] \label{co:FPL-uniform-noise}
Algorithm 1 applied for caching with exact requests has the following regret bound: 
\begin{align}
           \bar{\mathcal{R}}_{T}(\text{FPL})
& \leq 2\sqrt{2}\cdot  B \cdot \sqrt{C \cdot T}\ .
\end{align}
given that $C<N/2$.
\end{corollary}
\begin{IEEEproof}
We apply Theorem $1$ for the case where the decision set $\mathcal{X}$ is as in \eqref{eq:Capped-Simplex}, implying that the diameter $D$ is equal to $2\cdot C$ when $C<N/2$.
%G: isn't this always true also when C > N/2?
Also, the costs set $\bar{\mathcal{B}}$ is as in \eqref{eq:requests_set} and the unbiased estimator $\hat {\mathbf{r_t}}$ is always equal to the request $\mathbf{r_t}$. It follows that  $\mathcal{\bar{B}}= \hat{\mathcal{B}}$ and then, by definition of $\mathcal{\bar{B}}$, it follows that $\hat A=B$ and $\hat R=B$. Replacing the constants $\hat R, \hat A$ and $D$ in the result of Theorem $1$ we get our result. 
\end{IEEEproof}

In~\cite{bhattacharjee2020fundamental} Bhattacharjee et al. proposed an FPL-based algorithm with a Gaussian noise for the online caching problem and they proved the following bound on the regret (according to the regret definition in~\eqref{eq:regret}). 

\begin{theorem}\cite[Theorem 3]{bhattacharjee2020fundamental}
\label{th:FPL-gaussian-noise}
  For $\eta = \frac{1}{4\pi (\ln N)^{1/4}} \cdot \sqrt{\frac{T}{C}}$ and for $\gamma_t$ normal gaussians, with $r_0 = \eta \cdot \gamma_t$, the expected regret of FPL is given by: 
  \begin{align}
      \mathcal{R}_{T}(\text{FPL})  \leq 1.51 \cdot (\ln N)^{1/4} \cdot \sqrt{C\cdot T}\ .
  \end{align}
\end{theorem}

Since $\mathcal{\bar R}_T \le \mathcal{R}$ the regret bound is also valid for the weak regret defined in~\eqref{eq:pseudoregret}. In this view, our analysis presents two main novelties. First, our bound in Corollary~\ref{co:FPL-uniform-noise} is also valid in the case where the requests are batched, which is of practical interest since updating the cache at each request might be computationally impractical due to the high request rate. Second, even when the batch size $B$ is equal to 1, we provide a bound that does not depend on the catalogue size, and hence it will not diverge as $N$ goes to infinity. %Our analysis has advantage over state of the art FPL algorithm for caching in two dimensions. First, our bounds are also valid when requests are batched, which is of practical interest, since updating the cache at each time step might be unfeasible due to the high request rate. Second, even for the case when the batch size $B=1$, our regret bounds are tighter for a catalogue size $N\geq 13$. Moreover, \cite{bhattacharjee2020fundamental} bounds diverge as $N$ goes to infinity in contrast with our bounds that are independent of the catalogue size.

\subsection{NFPL for caching}
\label{ss:NFPL-Caching-Fixed}
In the caching problem, especially in cases where the request rate is very high~\cite{estan2002new}, the sample of the actual requests within each batch can allow the use of slower and cheaper memory. In what follows we take into account two different ways of sampling requests inside each batch of requests. First, we consider the case where the caching system samples a fixed number of requests from each batch. Second, we consider the case where each request of the batch is independently sampled with a specified probability.

{\noindent \textbf{Fixed number of samples}}. 
%For the caching problem, it is of interest to consider only a subset of requests at each batch of size $l<B$. This is beneficial as the rate by which counters are updated is smaller and hence it can be afforded to use a slower cheaper memory for storing counts for each object. 
%We consider then the setting where we have access a sample $l$ out of $B$ requests, chosen uniformly at random from the batch. If $s_t$ is the sequence of requests in the batch, with frequency count for each object inside the batch $r_t$, $\hat s_t$ is sub-sequence of $s_t$ with length $l<B$ and $\hat d_t$ is the frequency count for each object inside the batch $\hat s_t$ . The unbiased estimator in this case is given by: 
We study the setting where the caching system has access to a sample of $l < B$
%G: "b" instead of "l"?
requests uniformly chosen at random from the batch at each time-slot. Let $\mathbf{\hat d}_t$ denote the vector of requests for each file in the sampled batch. We then use the following unbiased estimator for $\mathbf{r}_t$:
\begin{equation}\label{e:fixed-batch}
        \mathbf{\hat{r}_{t}}  =   \frac{B}{l} \cdot  \mathbf{\hat{{d_t}}}: \; \E{\mathbf{\hat r_t}} = \mathbf{r_t}. \;
\end{equation}

Using NFPL in this setting, we obtain the following regret bound:
\begin{corollary}[Regret Bound NFPL with fixed size sub-batch]\label{co:NFPL-caching-fixed-subBatch}
      For $\eta = B \cdot \sqrt{\frac{T}{2\cdot C}}$, the expected regret of NFPL verifies: 
        \begin{align}
                 \bar{\mathcal{R}}_{T}(\text{NFPL}) \leq 2\sqrt{2} \cdot B \cdot \sqrt{C\cdot T}
        \end{align}
    
\end{corollary}
\begin{IEEEproof}
        We apply Theorem $1$ for the case where $\mathcal{X}$ is as in \eqref{eq:Capped-Simplex}, implying that the diameter $D$ is equal to $2\cdot C$ when $C<N/2$. Also, the costs set $\bar{\mathcal{B}}$ is as in \eqref{eq:requests_set} and the unbiased estimator $\hat {\mathbf{r_t}}$ is given in \eqref{e:fixed-batch}. Notice that in this case $\norm{\hat{\mathbf{r_t}}}_1 = B$ for every realization we deduce then that $\hat A = B$ and $\hat R = B$. Replacing the constants $\hat R, \hat A$ and $D$ in the result of Theorem $1$ we get our result. 
\end{IEEEproof}
\begin{remark}
The regret bound in Corollary \ref{co:NFPL-caching-fixed-subBatch} is independent from the sub-batch size $l$. However, we will show in Section~\ref{sec:experiments} that the smaller is the value of $l$, the higher is the variability in the cost of our algorithm.  
\end{remark}

{\noindent \textbf{Variable number of samples}}. Another approach is to consider a sub-batch where each request is independently sampled with probability $f>0$ at each iteration. In this case, the size of the sub-batch is a random variable and we consider the following unbiased estimator
%Another model, is to consider a sub-batch that samples each request with a probability $f>0$ at each time step, in this case the size of the batch is a random variable and the unbiased estimator $\hat r_t$ is expressed in this case as: 
\begin{equation}\label{e:estimator-rt-f}
    \mathbf{\hat {r}_t} = \frac{1}{f} \cdot \mathbf{\hat d}_t,
\end{equation}
where $\mathbf{\hat d}_t$ is defined as in \eqref{e:fixed-batch}. In this case, NFPL achieves the following regret bound:
\begin{corollary}[Regret Bound NFPL sampling probability $f$]\label{c:sampling}
      For $\eta = \frac{B}{f} \cdot \sqrt{\frac{T}{2\cdot C}}$, the expected regret of NFPL verifies: 
        \begin{align}
                 \mathcal{\bar{R}}_{T}(\text{NFPL}) \leq 2\sqrt{2} \cdot \frac{B}{f} \cdot \sqrt{C\cdot T}
        \end{align}
\end{corollary}
\begin{IEEEproof}
 We apply Theorem $1$ for the case where the decision set $\mathcal{X}$ is as in \eqref{eq:Capped-Simplex}, implying that the diameter $D$ is equal to $2\cdot C$ when $C<N/2$. Also, the costs set $\bar{\mathcal{B}}$ is as in \eqref{eq:requests_set} and the unbiased estimator $\hat {\mathbf{r_t}}$ is given in \eqref{e:estimator-rt-f}. Notice that in this case $\norm{\hat {\mathbf{r_t}}}_1 \leq \frac{B}{f}$ for very realization. It follows that $\hat A = \hat R = \frac{B}{f}$. Replacing the constants $\hat R, \hat A$ and $D$ in the result of Theorem $1$ we get our result. 
\end{IEEEproof}

\begin{remark}
    The bound in Corollary~\ref{c:sampling} shows the dependency on the sampling probability $f$. Surprisingly, we always have $\bar{\mathcal{R}}_{T} = \mathcal{O}(\sqrt{T})$ but as $f$ goes to $0$, the constant in our bound for the regret becomes larger.  
\end{remark}


% \begin{remark}
%  It seems that the difference between NFPL and FPL is the constant in the regret $\frac{1}{p}$. But NFPL has more variance, since the expectation is taken now over more randomness. 
% \end{remark}



% \begin{algorithm}[h] 
% \KwIn{$R,\; T,\; B, \; D_1$}
% \KwOut{Sequence of cached items: $\{x_t\}_{1}^{T}$}

% $\eta \gets \sqrt{\frac{R\cdot B \cdot T}{D_1}}$ \\ 
% $\textbf{costs} \gets \textbf{Unif}\left(\left[0, \eta\right], \mathbb{I}_{N\times N}\right)$ ,  \\ 
% \For{round $t=1,2,...,T$}{
% $x_t \gets M(costs)$ \\ 
% Observe sample $\hat r_t \sim \frac{1}{f} \textbf{Binom}(r_t,f,\mathbb{I}_{N\times N})$ \\
% $\textbf{costs} \gets \textbf{costs} + \hat r_t$
% }
% \label{alg:NFPL}
% \caption{Follow the Perturbed Leader with Uniform Noise (NFPL) for Caching}
% \end{algorithm}
% {\noindent}Algorithm \ref{alg:NFPL} only observes a sample of requests $\hat r_t$ such that each request is seen with probability $p$. This results in noisy frequency count.

==> Journal/Recovery_Files/background1.tex <==
We consider a single-cache system where requests for files are served locally by a cache of finite capacity or, in the case of file miss, by a remote server. This latter case implies a per-file dependent cost related to the file retrieval. Such a cost can represent the time needed to retrieve the file from the remote server, or a monetary cost due to the use of the network infrastructure. 
% Younes : Maybe it not necessary to specify the weights w_i  OK

{\noindent \bf Cache State}. The local cache has capacity $C \in \{1,\ldots,N\}$, and it stores the files entirely. The cache state at time $t$ is represented by the vector $\textbf{x}_t = [x_{t,i}]_{i\in \mathcal{N}}$ indicating the files missing in the cache, i.e., $x_{t,i} = 1$ if file $i$ is missing at time $t$. Such a vector belongs to the set
\begin{equation*}
\mathcal{X} = \left \{ x \in \{0,1\}^{N} | \sum_{i\in \mathcal{N}} x_{i} = N-C \right \}.
\end{equation*}
The set $\mathcal{X}$ is the capped simplex defined by the capacity constraint of the local cache.

{\noindent \bf Cache Updates}. Caching decisions are taken after  batch of $B$ requests has been cumulated, i.e., at each time-slot $t=1,\ldots,T$,
$B$ requests are collected from the users and the cache state is updated. The request process is represented as a sequence of vectors $\mathbf{r}_t = (r_{t,i} \in \mathbb{N}: i \in \mathcal{N})$ $\forall t$, where $r_{t,i}$ is the number of requests received for file $i$ at time $t$ in a file batch of size $B$. All the requests belong to the set
\begin{equation*}\label{eq:requests_set}
\mathcal{R} = \left \{ \mathbf{r}_t \in \mathbb{N}^N, t = 1, \dots, T | \sum_{i \in \mathcal{N}} r_{t,i} = B \right \}.
\end{equation*}
% Hence, we have
% \begin{equation}
%     \norm{\mathbf{r}_t}_{1} = B, \quad \norm{\mathbf{r}_t}_2 \leq B, \forall t \ .
% \end{equation}
{\noindent \bf Cost}. At each time-slot $t$, the caching system pays a cost equal to the number of requested files that are missing. Formally:
\begin{equation}\label{eq:cost}
\phi_{\mathbf{r}_t}(\mathbf{x}_t) = \scalar{\mathbf{r}_t}{\mathbf{x}_t}.
\end{equation}
% We have that: 
% \begin{align}
%     R &= \sup_{\mathbf{x},\mathbf{y}\in \mathcal{X}, t \in [T]} |\scalar{\mathbf{r}_t}{(\mathbf{x}-\mathbf{y})}| \leq B \cdot D_2 = \sqrt{2C}\cdot B \ .
% \end{align}
%Do we really need to define R ? 
For the sake of clarity, in what follows, for any vector $\mathbf{r}$, we indicate with $M(\mathbf{r})$ an arbitrary element of $\arg\min_{\mathbf{x}\in \mathcal{X}} \scalar{\mathbf{r}}{\mathbf{x}}$.
Furthermore, given a sequence of vectors $(\mathbf{r}_1, \dots, \mathbf{r}_t)$, we denote their aggregate sum as $\mathbf{r}_{1:t}\triangleq \sum_{s=1}^t \mathbf{r}_s$. 

\subsection{Online Caching}
Our caching problem falls in the \textit{Online Convex Optimization} framework~\cite{zinkevich2003online, hazan2016introduction}, where an agent (caching system) chooses an action $\textbf{x}_t$ from a convex set $\mathcal{X}$ at each time-slot $t$ before an adversary selects the cost function $\phi_{\mathbf{r}_t}$, i.e., the system changes the cache state before experiencing the cost. The cache state is determined by an online algorithm $\mathcal{A}$ that, at each time-slot $t$, computes the cache state $\textbf{x}_{t+1}$ for the next time-slot given the current state $\mathbf{x}_t$ and the costs seen so far $\{\mathbf{r}_{s}\}_{s=1}^{t}$. The main performance metric used to evaluate an online algorithm $\mathcal{A}$ is the regret:
%\begin{equation}\label{eq:regret}
%R_T(\mathcal{A}) = \sup_{\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}} \left \{\sum_{t=1}^T %f_{\mathbf{r}_t}(\mathbf{x}_t) - \sum_{t=1}^T f_{\mathbf{r}_t}(\mathbf{x}^*) \right \}
%\end{equation}.
\begin{equation}\label{eq:regret}
    \mathcal{R}_T = \sup_{\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}} \left \{\sum_{t=1}^{T} \scalar{\mathbf{r}_t}{\mathbf{x}_t} - \text{OPT}(1:T)\right \}.
\end{equation}
%Younes: Not sure if the point should be here, and I would prefer to mention x^{*} right away. 
This metric measures the difference the total cost incurred by $\mathcal{A}$ over a time horizon $T$ and the total cost of the static optimum $\text{OPT} = \scalar{\mathbf{r}_{1:T}}{M(r_{1:T})}$. %decision $\mathbf{x}^*$ in hindsight for any sequence of requests, i.e., $\mathbf{x}^* = \arg\min_{\mathbf{x} \in \mathcal{X}} \sum_{t=1}^T f_{\mathbf{r}_t}(\textbf{x})$. 
The supremum in~\eqref{eq:regret} indicates that the regret is compared against an adversary that generates requests trying to deteriorate the performance of the caching system.
% Younes: I do not know if maybe here we could talk about oblivious and adaptive, probably not the right place, because this only matters when the algorithm has randomness. I would also suggest to say instead that it holds for any sequence of requests. OK
In this setting, the main goal is the design of an online caching algorithm $\mathcal{A}$ that achieves sublinear regret, i.e., $R_T(\mathcal{A}) = o(T)$. This ensures that the designed algorithm behaves as the optimal static policy on average achieving zero average regret as $T$ increases.

\subsection{Follow the Perturbed Leader (FPL)}
In the OCO literature, one of the projection-free algorithms that achieve linear regret is the \textit{Follow the Perturbed Leader} (FPL) introduced by Vempala et al. in~\cite{kalai2005efficient}, and then studied in the caching framework by Bhattacharjee et al. in~\cite{bhattacharjee2020fundamental}.
%Younes: I would not say 0 regret  but sublinear regret. Most efficient might be a big claim. 
The algorithm is a smoothed version of the classic \textit{Follow the Leader} (FTL) algorithm~\cite{littlestone1994weighted} that greedily selects the next state minimizing the aggregate costs seen in the past, i.e., $x_{t+1}(\text{FTL}) = M(r_{1: t})$. %$\mathbf{x}_{t+1} = \arg\min_{\mathbf{x} \in \mathcal{X}} \sum_{\tau=1}^t f_{\mathbf{r}_{\tau}}(\mathbf{x})$. 
FTL algorithm is optimal when the cost functions are sampled from a stationary distribution, however, in the adversarial setting, the algorithm presents linear regret~\cite{de2014follow}. 
%The behaviour of FTL can be easily exploited by an adversary by always requesting all the files that are not stored in the current time-slot leading to a linear regret for the algorithm.
%Younes: Here we are talking about online convex optimization in general so I think it is a bit weird to go back to caching. I think maybe we could just cite a paper that shows FTL is not good OK

%Younes: Maybe this is the right time To introduce the notation M(r_{i:j}) OK
FPL algorithm improves the performance of FTL by adding an initial random noise vector $\mathbf{r}_0$ where each component of the vector is drawn from a uniform distribution independently. In this case, the update is the following:%in the range $\left[ -\eta , \eta\right]$ independently, where $\eta \in \mathbb{R}^+$. 
 \begin{equation}
     x_{t+1}(\text{FPL}) = M(r_{0:t}) \ .
 \end{equation}
As described in~\cite{bhattacharjee2020fundamental}, in the case of caching, the algorithm first samples a vector of random variables $\boldsymbol \eta$. Then, at every time-slot, it adds the random noise to 
the current cumulative cost vector $\mathbf{r}_{0:t}$. Finally, the algorithm caches $C$ files with the lowest perturbed cumulative cost at each time-slot.
As shown in~\cite{bhattacharjee2020fundamental}, FTPL provides optimal regret guarantees for the discrete caching problem. Furthermore, this algorithm is also computationally efficient with respect to other approaches such as \textit{Follow-the-Regularized-Leader} or the Online Gradient Descent (OGD) methods~\cite{paschos2020online}, since it requires a sorting operation instead of projection.
%Younes: Maybe here, we can just give the definition 
%Younes: We can here refer directly to OGD 




==> Journal/Recovery_Files/background2.tex <==
We consider a single-cache system in which file requests for a catalogue with $N$ files can either be served locally by a cache with finite capacity $C$ or, in the case of a file miss, by a remote server. 
%The latter scenario incurs a file-dependent cost associated with retrieving the file. This cost may represent the time needed to fetch the file from the remote server or a monetary expense due to the use of network infrastructure.
%G: WHY TALK ABOUT FILE-DEPENDENT COSTS IF LATER WE JUST LOOK AT THE MISS COST.

{\noindent \bf Cache State}. The local cache has a capacity $C \in \{1,\ldots,N\}$ and stores files in their entirety. The cache state at time $t$ is represented by the vector $\textbf{x}_t = [x_{t,i}]_{i\in \mathcal{N}}$, which indicates the files missing in the cache; that is, $x_{t,i} = 1$ if and only if file $i$ is not stored in the cache at time $t$. A feasible cache allocation is then represented by a vector in the set:

\begin{equation*}
\mathcal{X} = \left \{ x \in \{0,1\}^{N} | \sum_{i=1}^N x_{i} = N-C \right \}.
\end{equation*}

%The set $\mathcal{X}$ represents the capped simplex defined by the capacity constraint of the local cache.
%G: technically this is not the capped-simplex


{\noindent \bf Cache Updates}. Although caching policies are often assumed to update their state after each request, in high request regimes or when cache updates are computationally or communicationally expensive, the cache may update its state after receiving a batch of $B$ requests~\cite{salem2021no}.
We study caching policies in this more general setting and consider a time-slotted operation. At each time-slot $t=1,\ldots,T$,
$B$ requests are collected from the users and the cache state is updated. The request process is represented as a sequence of vectors $\mathbf{r}_t = (r_{t,i} \in \mathbb{N}: i \in \mathcal{N})$ $\forall t$, where $r_{t,i}$ is the number of requests received for file $i$ at time $t$ in a file batch of size $B$. All the requests belong to the set
\begin{equation*}\label{eq:requests_set}
\bar{\mathcal{R}} = \left \{ \mathbf{r}_t \in \mathbb{N}^N, t = 1, \dots, T | \sum_{i=1}^N r_{t,i} = B \right \}.
\end{equation*}

{\noindent \bf Cost}. At each time-slot $t$, the caching system pays a cost equal to the number file misses, i.e., the number of files that must be retrieved by the remote server. Formally:
\begin{equation}\label{eq:cost}
\phi_{\mathbf{r}_t}(\mathbf{x}_t) = \scalar{\mathbf{r}_t}{\mathbf{x}_t}= \sum_{i=1}^N r_{t,i} x_{t,i},
\end{equation}
where $\scalar{\mathbf{r}_t}{\mathbf{x}} \triangleq \sum_{i=1}^N r_{i} x_i$ denotes the scalar product of the two vectors $\mathbf{r}$ and $\mathbf{x}$.
% We have that: 
% \begin{align}
%     R &= \sup_{\mathbf{x},\mathbf{y}\in \mathcal{X}, t \in [T]} |\scalar{\mathbf{r}_t}{(\mathbf{x}-\mathbf{y})}| \leq B \cdot D_2 = \sqrt{2C}\cdot B \ .
% \end{align}
%Do we really need to define R ? 

For the sake of coinciseness, we introduce the following  notation. For any vector $\mathbf{r}$, we denote by $M(\mathbf{r})$ an arbitrary element of $\arg\min_{\mathbf{x}\in \mathcal{X}} \scalar{\mathbf{r}}{\mathbf{x}}$. Furthermore, given a sequence of vectors $(\mathbf{r}_1, \dots, \mathbf{r}_t)$, we represent their aggregate sum as $\mathbf{r}_{1:t}\triangleq \sum_{s=1}^t \mathbf{r}_s$.

\subsection{Online Caching}
%G: NO, THIS IS NOT TECHNICALLY CONVEX OPTIMIZATION, BECAUSE THE VARIABLE IS DISCRETE
Caching  may be framed as an \textit{online learning problem}~\cite{hazan2016introduction}, where an agent (the caching system) chooses an action $\textbf{x}_t$ from a set $\mathcal{X}$ at each time-slot~$t$ before an adversary selects the cost function $\phi_{\mathbf{r}_t}: \mathcal X \to \mathbb R$.
%, i.e., the system changes the cache state before experiencing the cost. 

The cache state is determined by an online algorithm $\mathcal{A}$ that, at each time-slot $t$, computes the cache state $\textbf{x}_{t+1}$ for the next time-slot given the current state $\mathbf{x}_t$ and the cost functions incurred so far, which, in our application, are  determined solely by the sequence of requests up to time~$t$, that is $\{\mathbf{r}_{s}\}_{s=1}^{t}$. 

The main performance metric used to evaluate an online algorithm $\mathcal{A}$ is the regret, for which two different definitions are available. The expected regret is defined as 
%\begin{equation}\label{eq:regret}
%\bar{\mathcal{R}}_T(\mathcal{A}) = \sup_{\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}} \left \{\sum_{t=1}^T %f_{\mathbf{r}_t}(\mathbf{x}_t) - \sum_{t=1}^T f_{\mathbf{r}_t}(\mathbf{x}^*) \right \}
%\end{equation}.
\begin{equation}\label{eq:regret}
    \mathcal{R}_T(\mathcal A) = \E{\sup_{\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}} \left \{\sum_{t=1}^{T} \scalar{\mathbf{r}_t}{\mathbf{x}_t} - \text{OPT}_T\right \}},
\end{equation}
where $\text{OPT}_T = \scalar{\mathbf{r}_{1:T}}{M(\mathbf{r}_{1:T})}$ is the minimum cost incurred under the request sequence $\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}$ by the optimal static allocation $\mathbf{x}^* = M(\mathbf{r}_{1:T})$, and the expectation is taken over all any random choice of the algorithm $\mathcal A$.
The expected regret quantifies then the performance gap over a time horizon $T$ between the algorithm $\mathcal{A}$  and best static cache allocation with hindsight.
%decision $\mathbf{x}^*$ in hindsight for any sequence of requests, i.e., $\mathbf{x}^* = \arg\min_{\mathbf{x} \in \mathcal{X}} \sum_{t=1}^T f_{\mathbf{r}_t}(\textbf{x})$. 
In contrast, the mean regret~\cite{belmega2018online} (also called pseudo-regret or weak regret) is defined as 
\begin{equation}\label{eq:pseudoregret}
    \bar{\mathcal{R}}_T(\mathcal A) = \sup_{\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}} \left \{ \E{\sum_{t=1}^{T} \scalar{\mathbf{r}_t}{\mathbf{x}_t}} - \text{OPT}_T\right \}.
\end{equation}
The interpretation remains analogous, but the mean regret involves comparing the \emph{expected} performance of algorithm $\mathcal A$ with that of the optimal static cache allocation. Applying Jensen's inequality leads one directly to conclude that $\bar{\mathcal{R}}_T \le  \mathcal{R}_T$. Our findings are articulated in terms of the mean regret, which we will henceforth refer to as just 'regret'.

Due to the supremum over all request sequences in~\eqref{eq:regret} and in~\eqref{eq:pseudoregret}, regret metrics do not make any assumptions about the nature of the request sequence (e.g., no statistical regularity). This means that the request sequence could be generated by an adversary seeking to degrade the performance of the caching system.
% Younes: I do not know if maybe here we could talk about oblivious and adaptive, probably not the right place, because this only matters when the algorithm has randomness. I would also suggest to say instead that it holds for any sequence of requests. OK

In this setting, one aims for an algorithm with sublinear regret, $\bar{\mathcal{R}}_T(\mathcal{A}) = o(T)$. These algorithms are commonly known as \emph{no-regret algorithms} since their time-average cost approaches the optimal static policy's cost as $T$ grows.

%G: WRITE SOMETHING ALONG THE FOLLOWING LINES:
%Online algorithms have regret can achieve a regret bound of at most $\sqrt{T}$~\cite{mcmahan2017survey}. 
%G: exactly the opposite, this is a lower bound for caching problem (cite sinha, it has the probabilistic method proof we discussed). I am not sure such result is in mcmahan, as it is not true for general online learning algorithm (bandit algorithm can have \log t). I do not have time to check this, also because I think such bounds are in terms of the expected regret rather than the mean regret.
Various algorithms, such as Online Gradient Descent (OGD) and Follow the Regularized Leader (FRL), can attain $\mathcal O(\sqrt{T})$-regret for caching problems~\cite{paschos2019learning,mhaisen2022online}. However, their cache update procedures necessitate projecting a tentative solution back onto the feasible set, which incurs $O(N^2)$ computational cost~\cite{wang2015projection}. %in the general case~\cite{wang2015projection} of batched requests~\cite{salem2021no}. %and $O(...)$ for OGD and FRL, respectively~\cite{wang2015projection,}. 
%G: check the projection cost in Tareq, I think it is smaller.
In the next section, we present a lightweight caching algorithm with $O(\sqrt{T})$-regret.

\subsection{Follow the Perturbed Leader (FPL)}
In the online learning literature, one of the projection-free algorithms that achieve sublinear regret is the \textit{Follow the Perturbed Leader} (FPL) introduced by Vempala et al. in~\cite{kalai2005efficient}, and then studied in the caching framework by Bhattacharjee et al. in~\cite{bhattacharjee2020fundamental}.
The algorithm is a smoothed version of the classic \textit{Follow the Leader} (FTL) algorithm~\cite{littlestone1994weighted} that greedily selects the next state minimizing the aggregate costs seen in the past, i.e., $x_{t+1}(\text{FTL}) = M(r_{1: t})$. %$\mathbf{x}_{t+1} = \arg\min_{\mathbf{x} \in \mathcal{X}} \sum_{\tau=1}^t f_{\mathbf{r}_{\tau}}(\mathbf{x})$. 
FTL algorithm is optimal when the cost functions are sampled from a stationary distribution, however, in the adversarial setting, the algorithm presents linear regret~\cite{de2014follow}. 
%The behaviour of FTL can be easily exploited by an adversary by always requesting all the files that are not stored in the current time-slot leading to a linear regret for the algorithm.
%Younes: Here we are talking about online convex optimization in general so I think it is a bit weird to go back to caching. I think maybe we could just cite a paper that shows FTL is not good OK

%Younes: Maybe this is the right time To introduce the notation M(r_{i:j}) OK
FPL algorithm improves the performance of FTL by adding an initial random noise vector $\mathbf{r}_0$ where each component of the vector is drawn from a uniform distribution independently. In this case, the update is the following:
%Younes: FPL does not necessarily use a noise that is uniform or exponential, so we can keep it general ? Like by choosing the right noise ?
%in the range $\left[ -\eta , \eta\right]$ independently, where $\eta \in \mathbb{R}^+$. 
 \begin{equation}
     x_{t+1}(\text{FPL}) = M(r_{0:t}) \ .
 \end{equation}
As described in~\cite{bhattacharjee2020fundamental}, in the case of caching, the algorithm first samples a vector of random variables $\boldsymbol \eta$. Then, at every time-slot, it adds the random noise to 
the current cumulative cost vector $\mathbf{r}_{0:t}$. Finally, the algorithm caches $C$ files with the lowest perturbed cumulative cost at each time-slot.
As shown in~\cite{bhattacharjee2020fundamental}, FTPL provides optimal regret guarantees for the discrete caching problem. Furthermore, this algorithm is also computationally efficient with respect to other approaches such as \textit{Follow-the-Regularized-Leader} or the Online Gradient Descent (OGD) methods~\cite{paschos2020online}, since it requires a sorting operation instead of projection.
%Younes: Maybe here, we can just give the definition 
%Younes: We can here refer directly to OGD 




==> Journal/Recovery_Files/conclusions2.tex <==
In this paper we studied, in an online caching framework, a variant of the classic Follow-the-Perturbed-Leader (FPL) in the case of imperfect knowledge of the requests. First, we provided a general framework to analyse FPL in case of noisy requests and then we studied the performance of our proposed algorithm (NFPL) in terms of regret. We showed that NFPL achieves the same regret guarantees of FPL with perfect knowledge of the requests, as far the requests' estimates are unbiased. Second, we experimentally showed that in case of particular non-stationary requests,
NFPL outperforms classic caching policies. Furthermore, different sampling methods have similar performance in both synthetic and real datasets. Future works involve the study of other online algorithms with imperfect knowledge of requests in the online caching framework.

==> Journal/Recovery_Files/intro1.tex <==
The use of caching techniques is becoming pervasive in many research fields related to computer systems. Ranging from the speed-up of CPUs' performance to the optimization of users' experience in CDNs~\cite{bektas2007designing}. The main goal in a caching system
is to choose the set of files to be stored in the cache in order to maximize the 
probability that a new file request is served locally avoiding the file retrieval from a remote server. With the constant increasing of network traffic due to 
the diffusion of new services such as virtual and augmented reality applications~\cite{chatzopoulos2017mobile}, or edge video analytics~\cite{ananthanarayanan2017real}, caching policies can greatly help in mitigating the issues related to the transportation of data in computer networks.

Caching policies have been studied under different assumptions on the request process 
for new files. The most recent one belongs to the online learning theory where the 
requests are thought to be selected by an adversary~\cite{bhattacharjee2020fundamental,li2021online,paschos2019learning}. With this assumption, starting from the work of Paschos et al.~\cite{paschos2019learning}, the online caching has been analysed under the lens of the \textit{Online Convex Optimization} (OCO) framework~\cite{zinkevich2003online}. In this context, the main metric of interest is the \textit{regret}, i.e., the difference between the cost incurred by a given online algorithms
%algorithm not algorithms right ? 
and the cost of the best static solution that has complete knowledge of future requests over a fixed time horizon. The main goal is to design \textit{no-regret} algorithms, i.e., online policies whose regret grows sublinearly with the length of the time horizon~\cite{paschos2019learning}.

Several online caching policies have been proposed in the literature, based on well-known online algorithms such as Online Gradient Descent (OGD)~\cite{paschos2019learning}, Follow-the-Regularized Leader (FTRL) or Follow-the-Perturbed-Leader (FPL)~\cite{mhaisen2022optimistic}. All these policies assume to have perfect knowledge of the received requests, however, when the request rate is very high~\cite{estan2002new} it is hard to get the actual requests and the requests seen by the caching system can be noisy. In this case, online caching policies should perform a sampling of the actual requests. This can let the caching system afford to use cheaper and slower memory to serve the requests (e.g., the count-min sketch techniques). In this paper we consider the FPL algorithm (one of the computationally less expensive algorithms) in the caching context and we extend it to deal with noisy requests. We show that even when we do not have a perfect knowledge of the requests we can adapt FPL to have the same performance of the case with perfect knowledge as far as we have an unbiased estimator of the request process. To the best of authors' knowledge this is the first work that consider noisy request in the online caching framework.

In this work we propose an extension of FPL, namely Noisy-Follow-the-Perturbed-Leader (NFPL), able to work on batches of requests where the requests within each batch can be noisy. Our main contributions are the following:\\
{\noindent \it 1)} We study the FPL algorithm in a batched case of caching and we give a new bound that does not depend on the catalogue size.\\
{\noindent \it 2)} We extend FPL to work with noisy requests and we analytically prove that it provides the same performance with respect to the case with perfect knowledge in expectation as far as it has an unbiased estimator of the requests. \\
{\noindent \it 3)} We experimentally show, both on stationary traces and real ones, that NFPL present similar behaviour with respect to the classic FPL and LFU and it outperforms the state-of-the art in non-stationary cases.





==> Journal/backgroundV1.tex <==
%\subsection{Online linear learning + FPL} 
\subsection{Online linear learning}
\label{ss:OnlineLearning_FPL}
%\paragraph{Online linear learning}
In the online linear learning setting, an agent sequentially makes decisions in~$T$ rounds. At each round~$t$, the agent selects a decision vector~$\mathbf{x}_t$ from a set~$\mathcal{X}\subset \mathbb{R}^{N}$ and then observes a cost vector $\mathbf{r}_t$ from a set $\mathcal{B}\subset \mathbb{R}^{N}$. The agent then incurs a loss $\langle \mathbf{x}_t, \mathbf{r}_t \rangle$. In this context, the metric of performance for an algorithm $\mathcal{A}$ selecting a decision vector $\mathbf{x}_{t} = {\mathcal{A}}(\mathbf{r}_1,\ldots, \mathbf{r}_{t-1}, \mathbf{x}_{t-1})$ is the regret defined as follows, 
\begin{equation}
    \mathcal{R}_T(\mathcal A) = \sup_{\{\mathbf{r}_1,\ldots,\mathbf{r}_T\}} \left \{ \E{\sum_{t=1}^{T} \scalar{\mathbf{r}_t}{\mathbf{x}_t}} - \min_{\mathbf{x}\in \mathcal{X}} \langle \mathbf{x}, \sum_{t=1}^{T} \mathbf{r}_t\rangle\right \}\; ,
\label{eq:regret}
\end{equation}
 where $\scalar{\mathbf{r}}{\mathbf{x}} \triangleq \sum_{i=1}^N r_{i} x_i$ denotes the scalar product of the two vectors $\mathbf{r}$ and $\mathbf{x}$. 
 %For any vector~$\mathbf{r}$, we denote by $M(\mathbf{r})$ an arbitrary element of $\arg\min_{\mathbf{x}\in \mathcal{X}} \scalar{\mathbf{r}}{\mathbf{x}}$. Furthermore, given a sequence of vectors $(\mathbf{r}_1, \dots, \mathbf{r}_t)$, we represent their aggregate sum as $\mathbf{r}_{1:t}\triangleq \sum_{s=1}^t \mathbf{r}_s$.

The regret then quantifies the performance gap over a time horizon $T$ between the algorithm $\mathcal{A}$ and the best static solution with hindsight. Given the supremum taken over all the cost sequences in~\eqref{eq:regret}, it is evident that the regret metric refrains from making any assumptions regarding the characteristics of the cost sequence, such as any inherent statistical regularity. The cost sequence may be thought to have been generated by an adversary seeking to degrade the agent's performance. In this setting, the goal is to have an algorithm with sublinear regret, $\mathcal{R}_T(\mathcal{A}) = o(T)$. These algorithms are commonly known as \textit{no-regret} algorithms since their time-average cost approaches the optimal static policy cost as $T$ grows.

\subsubsection{FPL}

FPL serves as a refined version of the traditional Follow-the-Leader (FTL) algorithm~\cite{littlestone1994weighted} which greedily selects the state that would have minimized the past cumulative cost, i.e., $\mathbf{x}_{t+1}(\text{FTL}) = M(\mathbf{r}_{1:t})$. Where i) $M(\mathbf{r})$ denotes an arbitrary element of $\arg\min_{\mathbf{x}\in \mathcal{X}} \scalar{\mathbf{r}}{\mathbf{x}}$ for any vector~$\mathbf{r}$, and ii)  $\mathbf{r}_{1:t}\triangleq \sum_{s=1}^t \mathbf{r}_s$ represents the aggregate sum of a given sequence of vectors $(\mathbf{r}_1, \dots, \mathbf{r}_t)$. 

Although FTL proves optimal when cost functions are sampled from a stationary distribution, it unfortunately produces linear regret in adversarial settings~\cite{de2014follow}. The FPL algorithm improves the performance of FTL by incorporating a noise vector $\boldsymbol{\gamma}_t$ at each time step $t$.
The components of these vectors are independent and identically distributed random variables (i.i.d.), pulled from a distinct distribution (such as the uniform and exponential distributions in~\cite{kalai2005efficient}, and the Gaussian distribution in~\cite{abernethy2014online}). The update process unfolds similarly to FTL:
\begin{equation}
    \label{e:fpl_update}
     \mathbf{x}_{t}(\text{FPL}) = M(\mathbf{r}_{1:t-1}+\boldsymbol{\gamma}_{t}) .
 \end{equation}
Let~$D$ be the diameter of the set~$\mathcal{X}$, i.e., $D=\sup_{\mathbf{x},\mathbf{y}\in \mathcal{X}} \norm{\mathbf{x}-\mathbf{y}}_1$, $A$ be a bound on the norm $1$ of vectors in $\mathcal{B}$, and $R$ be a bound on $\langle \mathbf{x},\mathbf{r} \rangle$ for any $(\mathbf{x},\mathbf{r})\in \mathcal{X}\times \mathcal{B}$.

\begin{theoremSp}\cite[Thm. 1.1]{kalai2005efficient}
%When $\boldsymbol{\gamma}_{t+1}$ is sampled from a multivariate uniform distribution with uncorrelated components, constrained within the range $[0, \eta]^N$, with $\eta = \sqrt{RAT/D}$, then:
When $\boldsymbol{\gamma}_{t+1}$ is sampled from a multivariate uniform distribution with independent components over $[0, \eta]^N$, with $\eta = \sqrt{RAT/D}$, then:
\begin{align}
\mathcal{R}_T(\texttt{FPL}) \leq 2\sqrt{RADT}.
\end{align}
\end{theoremSp}

Most of the proposed no-regret algorithms within the online learning domain assume the convexity of both the objective function and the solution space to achieve proper guarantees in terms of regret. %However, among the online learning algorithms, 
The FPL algorithm %, is a notable methodology that performs a smooth perturbation of the cost vector. It 
has been shown to achieve sublinear regret even with non-convex (e.g., discrete) state space. It achieves optimal regret guarantees even under multiple distributions of the noisy vector $\gamma_t$,%for the perturbation of the cost vector, 
 as shown in~\cite{kalai2005efficient}.

\begin{table}
\centering
\caption{Computational complexity of a single iteration of online algorithms applied to caching.}
\begin{tabular}{p{0.30\columnwidth}p{0.25\columnwidth}p{0.30\columnwidth}}
\hline
{\bf Algorithm} & {\bf No-Batch} & {\bf Batch} \\
\hline
\hline
FPL & $O(\log C)$ & $O(N\log N)$ \\
%\hline
OGD & $O(N)$ & $O(N^2)$ \\
%\hline
OMD & $O(C)$  & $O(N)$\\
\hline
\end{tabular}\label{tab:Complexity}
\end{table}



% \subsection{Caching and Online Learning\color{black}}



\subsection{Caching and online learning}

Caching can be framed as an online learning problem~\cite{paschos2019learning}. An agent, i.e., the caching system with a cache of size $C$, chooses an action~$\mathbf{x}_t$, representing the cache state, from the set~$\mathcal{X}$ (representing all the feasible cache allocations) at each time slot~$t$ before an adversary reveals a request vector~$\mathbf{r}_t$%from the set $\mathcal{B} = \left \{ \mathbf{r}_t \in \mathbb{N}^N, t = 1, \dots, T | \sum_{i \in \mathcal{N}} r_{t,i} = B \right \}$
. The cache state is determined by an online algorithm $\mathcal{A}$ that, at each time slot $t$, computes the cache state $\mathbf{x}_{t+1}$ for the next time slot given the current state $\mathbf{x}_t$ and the sequence of requests up to time~$t$, that is~$\{\mathbf{r_{s}}\}_{s=1}^{t}$. The main performance metric used to evaluate an online caching algorithm $\mathcal{A}$, that updates the cache state $\mathbf{x}_{t}$ at each time step $t$, is the regret as defined in~\eqref{eq:regret}.

\textbf{Time complexity}. Various algorithms, such as Online Gradient Descent (OGD), Follow-the-Perturbed-Leader (FPL), and Online Mirror Descent (OMD), can attain $\mathcal O(\sqrt{T})$-regret for caching problems~\cite{paschos2019learning,mhaisen2022optimistic,si2023no}. However, one of the main concerns for online caching algorithms is represented by their computational time complexity that often hampers their adoption in practice. Table~\ref{tab:Complexity} summarizes the time complexity of these algorithms. For OGD and OMD,
the cache update procedures require a computationally expensive projection of a tentative solution back onto the feasible set $\mathcal X$. For OGD, Such an operation requires $O(N)$ iterations (where $N$ is the size of the entire file catalog) in case the cache is updated after receiving each single request (\textit{no-batch}), and $O(N^2)$ in case the cache is updated after collecting a batch of requests (\textit{batch)}~\cite{paschos2020online}. A recent work~\cite{carra2024online} showed that a logarithmic time complexity in the catalog size can be achieved by an online gradient-based caching policy (with no regret) by relaxing the cache constraint capacity and satisfying it only in expectation. As shown in~\cite{si2023no}, OMD algorithms achieve $O(N)$ in the batch case, and $O(C)$ in the no-batch case. It is worth mentioning that the aforementioned works have tackled the problem of fractional caching, where fractions of items can be stored in the cache. An additional routine of complexity $O(N)$~\cite{si2023no} is further needed to build a discrete cache state starting from a fractional one. As discussed in~\cite{mhaisen2022optimistic}, a perturbation-based smoothing adopted in FPL can avoid projections resulting in a time complexity of $O(N\log N)$ in the batched case due to the sorting of the items, and $O(\log C)$ in the \textit{no-batch} case. Indeed, in the latter case, just one item is inserted in the cache and, with a heap structure to keep track of the top $C$ items, the cost for updating the cache is $O(\log C)$~\cite{bhattacharjee2020fundamental}.
%Furthermore, we show that \texttt{NFPL} enjoys $O(1)$ amortized time complexity as the number of requests increases.}

\vspace{3mm}
\subsubsection{FPL in caching} 
Given its optimal guarantees, i.e., sublinear regret, and its low time complexity, we focus on FPL. The algorithm has been introduced in the caching context in~\cite{bhattacharjee2020fundamental}. The authors proved regret guarantees for FPL applied to caching under perfect knowledge of the requests. Furthermore, for the caching problem, they have obtained tighter bounds than what would have followed by directly applying the results from~\cite{CohenFPLStructruedLearning15}.
%Furthermore, they have not just applied the results from~\cite{abernethy2014online}, but they have improved the regret bounds for the caching problem. We report the result here for completeness.

\begin{theoremSp}\cite[Thm. 3]{bhattacharjee2020fundamental}
\label{th:FPL-gaussian-noise}
FPL applied to the caching problem with learning rate $\eta=\frac{1}{4\pi (\ln{N})^{1/4}} \sqrt{\frac{T}{C}}$, and noise vectors $\{\boldsymbol{\gamma}_t\}_{1}^{T}$, where $\boldsymbol{\gamma}_t/\eta$ is drawn from a standard multivariate normal distribution, has sublinear regret. More specifically
  \begin{align}
        \label{e:bound_bhattacharjee}
      \mathcal{R}_{T}(\text{FPL})  \leq 1.51 (\ln N)^{1/4} \cdot \sqrt{CT}.
  \end{align}
\end{theoremSp}

As shown in~\cite{bhattacharjee2020fundamental}, FPL provides asymptotically optimal regret guarantees in terms of $C$ and $T$, for the discrete caching problem. Moreover, the cache update, as specified in equation~\eqref{e:fpl_update}, involves storing the files that correspond to the largest elements of the vector $\mathbf{n}(t-1)+\boldsymbol{\gamma}_{t}$. %FPL cache update necessitates then a sorting operation.
%Notably, its computational complexity of $\mathcal O(N \log N)$ is less taxing than the projection step required by either the FRL or OGD algorithms, as highlighted in~\cite{mhaisen2022optimistic}.

In this work we are not taking into account fetching costs. Some work, such as~\cite{prakash2023regret}, presents a variant of FPL that considers the fetch costs of the requests achieving sublinear regret in case of adversarial requests. However, the case of partial observations of the requests is not considered.
%In~\cite{prakash2023regret}, a variant of FPL is presented to handle the service and the fetch costs of the requests. Their solution presents sublinear regret in case of adversarial requests. However, they assume that each item can be partially stored in the cache allowing fractional values of each component of the cache state. In our work, on the other hand, we assume that each item is entirely stored in the cache.

To the best of our knowledge, two works~\cite{liu2022learning,BuraPartial_Obser_caching_TON22} have studied the online caching problem with partial observation of the requests. Both works consider a scenario different than ours, where the caching system is only aware of requests for files it already stores. Bura et al.~\cite{BuraPartial_Obser_caching_TON22} have related the partial observation regime to a multi-armed bandit problem where actions, i.e., the item placement, are taken to learn the value of pulling different arms. On the other hand, Liu et al.~\cite{liu2022learning} propose an \texttt{FPL}-based caching policy that has sublinear regret for arbitrary requests for items already stored in the cache, and quadratic time complexity in the size of the catalog. In contrast, our solution is free from such computationally demanding operations, and achieves sublinear regret with no statistical assumptions on the request sequence.

%, though, in comparison to the basic \texttt{FPL} caching policy, at each step, their algorithm necessitates an additional geometric sampling operation whose time complexity scales as~$\mathcal{O}(N)$. In contrast, our solution is free from such computationally demanding operations and achieves sublinear regret with no statistical assumptions on the request sequence. 

%Unfortunately, the caching policy of Bura et al.~\cite{BuraPartial_Obser_caching_TON22} performs as well as the optimal static policy with full knowledge of the requests solely if the request process is stationary. On the other hand, Liu et al.~\cite{liu2022learning} propose an \texttt{FPL}-based caching policy that has sublinear regret for arbitrary requests for items already stored in the cache, though, in comparison to the basic \texttt{FPL} caching policy, at each step, their algorithm necessitates an additional sampling operation whose time complexity scales as~$\mathcal{O}(\sqrt{T})$. In contrast, our solution is free from such computationally demanding operations, and achieves sublinear regret with no statistical assumptions on the request sequence.}



% In the next section, we present a lightweight caching algorithm with $\mathcal{O}(\sqrt{T})$-regret.


%whose $\mathcal O(N \log N)$ is less demanding than 
%. This operation is computationally less demanding ($\mathcal $)than 
%the projection step required by the FRL or OGD algorithms~\cite{bhattacharjee2020fundamental}.




==> Journal/introFF.tex <==
Caching techniques are extensively employed in computer systems, serving various purposes such as accelerating CPU performance~\cite{tse1998cpu} and enhancing user experiences in content delivery networks (CDNs)~\cite{bektas2007designing}. The primary objective of a caching system is to carefully choose files for storage in the cache to maximize the proportion of file requests that can be fulfilled locally. This approach effectively minimizes the dependence on remote server retrievals, which can be costly in terms of delay and network traffic.
The presence of caching systems facilitates more efficient data delivery in network traffic and leads to enhanced overall system performance, especially with the widespread adoption of traffic-intensive applications such as virtual and augmented reality~\cite{chatzopoulos2017mobile}, or edge video analytics~\cite{ananthanarayanan2017real}.

Caching policies have been thoroughly investigated under numerous assumptions concerning the statistical regularity of file request processes~\cite{IRM,traverso2013temporal}. However, real-world request sequences tend to deviate from these theoretical models, especially when aggregated over small geographic areas~\cite{leconte2016placing}. This deviation has inspired the exploration of online learning algorithms, beginning with the work of Paschos et al.~\cite{paschos2019learning}, which applied the Online Convex Optimization (OCO) framework~\cite{zinkevich2003online} to caching. These algorithms exhibit robustness to varying request process patterns, as they operate under the assumption that requests may be generated by an adversary. 



In this context, the main metric of interest is the \emph{regret}, which is the difference between the cost---e.g., the number of cache misses---incurred by a given online caching algorithm
and the cost of the optimal static cache allocation with hindsight, i.e., with knowledge of the future requests over a fixed time horizon. In this framework, the primary objective is to design \emph{no-regret} algorithms, i.e., online policies whose regret grows sublinearly with the length of the time horizon~\cite{paschos2019learning}.

Several online caching policies have been proposed in the literature, drawing on well-known online algorithms such as Online Gradient Descent (OGD)~\cite{paschos2019learning}, Follow-the-Regularized-Leader (FRL)~\cite{mhaisen2022online} or Follow-the-Perturbed-Leader (FPL)~\cite{mhaisen2022optimistic}. The latter is especially promising, as cache updates can be performed without the need for computationally intensive projection operations over the set of feasible cache states.


% No-regret caching policies have  been studied under the assumption that the cache has perfect knowledge of each request (the only exception we are aware of is~\cite{liu2022learning} discussed below). However, in practical scenarios, the cache may only have access to noisy estimates of the number of requests for each file during a given time window. This can occur due to memory constraints necessitating the use of approximate sketches for counting requests~\cite{einziger2017tinylfu,mazziane2022analyzing} and/or to the high request rate forcing the sampling of the request sequence~\cite{wang2020stcs}.
% % (each request is served but the corresponding counter is not necessarily updated)
% A partial observation regime for requests in online caching is described in~\cite{liu2022learning}, however, the work just considers the case where the caching system is only aware of the requests for already-cached files. This can be seen as a particular case of the most general one of noisy requests considered in our study.


\ff{\textbf{Motivation}. \ding{202} Many of these online algorithms achieve asymptotically optimal regret bounds~\cite{bhattacharjee2020fundamental}, however they assume a full knowledge of the requests, i.e., the caching system is able to observe each content request coming into the system. In some relevant practical cases, such an assumption is not verified, with the cache system that does not have a complete view of the requests to be served. %, especially in cases where the decision on the cache update and the receiving of requests are two decoupled operations. 
%For example, in wireless content delivery networks~\cite{FEMTOCaching13TIT}, a central base station (BS) is charge of deciding which content to store in each single cache in the network. The requests received from all the single caches across the network are sent to the BS. In this case, the BS may not have a complete knowledge of all the requests received by the caches in the network due to communication losses. Second \ding{203}, when dealing with a vast file catalog and/or a high request rate, a cache might have to depend on noisy information. For instance, limited availability of high-speed memory can necessitate the use of approximate counters based on hash functions~\cite{einziger2017tinylfu}. Alternatively, request sampling might be employed to decrease the frequency of counter updates~\cite{li2016full}. Third \ding{204}, most of these online learning solutions involve computationally-expensive operations that are performed at each new request to update the contents stored in the cache. This can be particularly constraining for computationally-limited resources.}
%Caching policies, including no-regret ones,  make admission and eviction decisions based on information from the request sequence. This can include factors such as the number of past requests for each file or a list of the most recently requested files. However, when dealing with a vast file catalog and/or a high request rate, a cache might have to depend on noisy information. For instance, limited availability of high-speed memory can necessitate the use of approximate counters based on hash functions~\cite{einziger2017tinylfu,mazziane2022analyzing}. Alternatively, request sampling might be employed to decrease the frequency of counter updates~\cite{li2016full}.
For example, in wireless content delivery networks~\cite{FEMTOCaching13TIT}, there are different caches (helpers) displaced over the network to satisfy users' requests and central base stations take decisions on the updates of the caches' states. Given the limited transmission range between caches and base stations, it may be difficult to transmit all the requests resulting the base stations to have partial knowledge of all the requests received by the helpers. %The partial knowledge of the requests can be seen as a sampling process on the complete sequence of requests as shown in~\cite{mazziane2023no}. This can be achieved by adding some noise to the original vector of the requests.
%Second \ding{203}, when dealing with a vast file catalog and/or a high request rate, a cache system might rely on requests' sampling processes. For instance, limited availability of high-speed memory can necessitate the use of approximate counters based on hash functions~\cite{einziger2017tinylfu}. Alternatively, request sampling might be employed to decrease the frequency of counter updates~\cite{li2016full}. 
\ding{203} Furthermore, most of these online learning solutions involve computationally-expensive operations that are performed at each new request to update the contents stored in the cache. This can be particularly constraining for computationally-limited resources. One approach to solve this issue is to update the cache state after collecting a batch of requests in order to amortize the update cost~\cite{salem2021no,FaticantiFRL24}. However, the higher is the batch size and the higher is the regret achieved by online algorithms. In this paper we show that sampling the requests can be an effective approach to balance such a trade-off.}

\ff{We address the issues above by proposing Follow-the-Perturbed-Leader-based (FPL) algorithm that does not take into account all the requests. To the best of our knowledge, this is the first algorithm that works with a partial knowledge of the requests. Indeed, in~\cite{liu2022learning} the authors propose a partial-knowledge setting but they only consider requests for contents already stored in the cache. Furthermore we propose the first caching policy with constant time complexity. As we will show, to prove such a result, applying results from the online learning literature to the caching problem is not enough. }

%Surprisingly, much of the existing literature on no-regret caching policies overlooks these practical constraints. Typically, these studies operate under the assumption that caches have exact knowledge of the request sequences or of its summaries. A notable exception is the work presented in~\cite{liu2022learning}. However, it exclusively examines the scenario in which the cache is only aware of requests for files it already contains.

 %and noisy request estimates. 
\ff{\textbf{Contributions.} %In this paper, we bridge this gap by 
We propose an FPL-based algorithm that can be specialised according to the specific joint distribution of the noise for sampling the requests. The proposed solution show guarantees on both the regret and computational complexity. From the regret's point of view, we prove that it is possible to have no-regret caching strategies also in cases where not all the requests are completely observable. For the computational complexity we proved that there exist FPL-variants with a reduced amortized complexity with respect to the standard approach.
%We propose two variants of the FPL algorithm---renowned for its computational efficiency and no-regret properties---to manage partial information of the requests. The proposed solutions show guarantees on both the regret and the computational complexity. From the regret's point of view, we prove that it is possible to have no-regret caching strategies also in cases where not all the requests are completely observable. For the computational complexity we proved that there exist FPL-variants with a reduced amortized complexity with respect to the standard approach. 
We extend our preliminary work~\cite{mazziane2023no} and, more in details, the main contributions of this paper are the following:
\begin{itemize}
\item We modify the FPL algorithm to work with samples of the requests and prove that the algorithm maintains sublinear regret for all the specific joint distribution of the noise. In particular, with a probability $p$ of sampling from the requests we obtain a~$\mathcal{O}(\frac{\sqrt{T}}{p})$ regret.
%\item We modify the FPL algorithm to handle noisy request estimates and prove that, under specific conditions on the estimator, the algorithm maintains sublinear regret. We refer to this extended version as Noisy-Follow-the-Perturbed-Leader (NFPL).
%\item We analyse the performance of NFPL in two possible propose two variants of the NFPL algorithm for the caching problem, namely, NFPL-Fix and NFPL-Var, where the requests estimator uses sampling. We prove that NFPL-Fix and NFPL-Var have sublinear regret.   
\item We prove a new regret bound for the classic FPL caching policy that is independent of the catalog size.
%\item We propose a new variant of FPL, namely Noisy-Follow-the-Lazy-Leader (NFLL), that updates the cache each $O(\sqrt{T})$ requests while keeping the same sublinear regret guarantees. Furthermore, the time complexity of such algorithm is $O(1)$ as $T \rightarrow +\infty$.
\item For each of the specific joint distribution of the noise we have different time complexities that outperforms the complexity of the standard algorithms. In particular, we show that the time complexity of the general algorithm is $O(1)$ as $T \rightarrow +\infty$.
\item We show how sampling the requests leads to a trade-off between the regret and the amortized time complexity in scenarios where batching, i.e., updating the cache after a specific number of requests, can not be used.  
\item We show through experimental analysis the advantage of the proposed algorithm over classical caching policies. %We also evaluate the impact of the sampling rate on the performance of NFPL-Fix and NFPL-Var.  
\end{itemize}}

\ff{The paper is organized as follows. We give background details and discuss the related work in Section~\ref{sec:bacground}. The definition of the problem we are tackling is defined in Section~\ref{s:Caching-problem}. Section~\ref{sec:extending} describes the extensions of FPL to deal with partial knowledge of the requests~\ref{sec:extending}. The proofs of the guarantees in terms of regret and time complexity are showed in Section~\ref{sec:ProofThMain}. Experimental results are presented in Section~\ref{sec:experiments}. Finally, Section~\ref{sec:conclusions} concludes the paper.}


%\begin{itemize}
%    \item With respect to the conference paper, we introduce three variants of the \texttt{NFPL} algorithm previously proposed. Interestingly, for one of these variants, we show for the first time that it is possible to simultaneously achieve a regret of $\mathcal{O}(\sqrt{T})$ and an amortized time complexity of $\mathcal{O}(1+ \frac{1}{\sqrt{T}})$, ignoring dependencies on the cache capacity.  

%    \item We show how sampling the requests leads to a trade-off between the regret and the amortized time complexity in scenarios where batching, i.e., updating the cache after a specific number of requests, can not be used.  
%\end{itemize}


==> Journal/methodology.tex <==
\subsection{Methodology}






The proofs of the no-regret property of previously proposed caching policies~\cite{bhattacharjee2020fundamental,paschos2020online,si2023no,mhaisen2022online,FaticantiFRL24}, when all past requests are observed, rely on advances in Online Optimization, e.g., Online Convex Optimization (OCO)~\cite{hazan2016introduction}, where loss functions are revealed sequentially, and the goal is to dynamically update decisions to minimize the total sum of these loss functions. In the simplest caching scenario, the decision is to select a subset of files to store, and the loss function is binary and determined by the requested file, modeling the cost due to a miss. On the other hand, the proofs of the no-regret caching policies when only requests for cached files are observed leverage results related to the \textit{Combinatorial Semi-Bandits} framework~\cite{FPLWithGR/jmlr/NeuB16}. 




 Online Convex Optimization (OCO) or Combinatorial Semi-Bandits frameworks do not directly capture the partial observability regime considered in this paper. Instead, this regime is related to less explored domains of the online optimization literature, known as \textit{selective sampling}~\cite{adaptiveSelectiveExperts24} or \textit{label-efficient forecasters}~\cite{expertWithPartialTruth05}, where the objective is to reduce the frequency with which loss functions are observed. Still, most existing algorithms in this restricted setting focus on the well-known \textit{expert}'s problem. In this paper, we adapt the \texttt{FPL} online learning algorithm to this restricted setting to achieve sublinear regret in a broader class of online linear learning problems where the loss functions are linear. The caching problem is a specific instance within this family of problems, allowing us to prove the regret guarantees of \texttt{NFPL}. 
